Bayesian Inference of Tissue Heterogeneity for Individualized Prediction of Glioma Growth

Reliably predicting the future spread of brain tumors using imaging data and on a subject-specific basis requires quantifying uncertainties in data, biophysical models of tumor growth, and spatial heterogeneity of tumor and host tissue. This work introduces a Bayesian framework to calibrate the spatial distribution of the parameters within a tumor growth model to quantitative magnetic resonance imaging (MRI) data and demonstrates its implementation in a pre-clinical model of glioma. The framework leverages an atlas-based brain segmentation of grey and white matter to establish subject-specific priors and tunable spatial dependencies of the model parameters in each region. Using this framework, the tumor-specific parameters are calibrated from quantitative MRI measurements early in the course of tumor development in four rats and used to predict the spatial development of the tumor at later times. The results suggest that the tumor model, calibrated by animal-specific imaging data at one time point, can accurately predict tumor shapes with a Dice coefficient > 0.89. However, the reliability of the predicted volume and shape of tumors strongly relies on the number of earlier imaging time points used for calibrating the model. This study demonstrates, for the first time, the ability to determine the uncertainty in the inferred tissue heterogeneity and the model predicted tumor shape.

==> Makefile <==
all:	all_texs

clean: clean_texs clean_exec

clean_texs:
	rm -f *.aux
	rm -f *.log
	rm -f *.dvi
	rm -f *.toc
	rm -f *.blg
	rm -f *.bbl
	rm -f mri_prediction*.ps
	rm -f *.out
	rm -f *.nav
	rm -f *.snm
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind	
	rm -f *.fdb_latexmk
	rm -f *.fls	
	rm -f *.synctex.gz

clean_exec:
	rm -f *~

#OBJS_convert = \
#	rawfigs/xyz.eps \
#	rawfigs/abc.eps

# $(OBJS_convert)

all_texs:
	pdflatex 	mri_prediction.tex
	pdflatex 	mri_prediction.tex
	bibtex mri_prediction
	pdflatex 	mri_prediction.tex
	pdflatex 	mri_prediction.tex	
	

.SUFFIXES: .eps .png .jpg

%.eps: %.png
	convert $< $(basename $<).eps

%.eps: %.jpg
	convert $< $(basename $<).eps

